A Practical Theory of Generalization in Selectivity Learning

Query-driven machine learning models have emerged as a promising estimation technique for query selectivities. Yet, surprisingly little is known about the efficacy of these techniques from a theoretical perspective, as there exist substantial gaps between practical solutions and state-of-the-art (SOTA) theory based on the Probably Approximately Correct (PAC) learning framework. In this paper, we aim to bridge the gaps between theory and practice. First, we demonstrate that selectivity predictors induced by signed measures are learnable, which relaxes the reliance on probability measures in SOTA theory. More importantly, beyond the PAC learning framework (which only allows us to characterize how the model behaves when both training and test workloads are drawn from the same distribution), we establish, under mild assumptions, that selectivity predictors from this class exhibit favorable out-of-distribution (OOD) generalization error bounds. These theoretical advances provide us with a better understanding of both the in-distribution and OOD generalization capabilities of query-driven selectivity learning, and facilitate the design of two general strategies to improve OOD generalization for existing query-driven selectivity models. We empirically verify that our techniques help query-driven selectivity models generalize significantly better to OOD queries both in terms of prediction accuracy and query latency performance, while maintaining their superior in-distribution generalization performance.

==> response/summary.tex <==
\section*{Revision Summary}
Dear VLDB Reviewers and Meta-Reviewer,

Please find the revision of our submission to VLDB 2025: \emph{A Practical Theory of Generalization in Selectivity Learning}. The paper has been revised thoroughly to address the reviewers’ comments, with modified text highlighted in \textcolor{blue}{blue}. We would like to express our gratitude to the reviewers for their constructive and insightful comments. We summarize major revision items for easy reference.
\begin{itemize} [leftmargin=*]
    \item \textbf{Presentation Improvements (M1-M2)}. We have addressed textual issues and inconsistencies, and have \emph{extensively} revised Section~\ref{section.preliminaries} to make the theoretical discussions easier to understand, in accordance with R2's comments.
     \item \textbf{Theoretical Clarifications (M3-M6)}. We have clarified our prose to address the four theoretical concerns raised by R1.
     \item  \textbf{Implementation Details (M7)}. We have provided details about our implementation steps (\textit{e.g.,} data preprocessing, model training and prediction) of our approaches ($\textsc{NeuroCDF}$ and $\textsc{SeConCDF}$), in accordance with R2's comments.
     \item  \textbf{Experimental Evaluation (M8-M11)}. Apart from including detailed inference and training times for the proposed models, we have added comparisons with Robust-MSCN~\cite{negi2023robust}, in accordance with R2's comments. Moreover, in accordance with R3's comments, we also added another real-world dataset/workload from the CEB benchmark~\cite{ceb} to assess robustness and generalization over greater numbers of joins. The new workload contains 9-way joins, which is much larger than the 5-way joins we considered in the first draft. We also provided per-query performance for the new experiment.
      \item  \textbf{Model Adaptation and Interpretability (M12).} We discussed the possibilities of adapting NeuroCDF to XGBoost and why NNs were our primary choice, in accordance with R3's comments.
    
\end{itemize}


\section*{\uppercase\expandafter{\romannumeral1.}\quad RESPONSE TO META REVIEWER}

The meta-reviewer requested that we address the individual reviewers' comments. In addition to the summary above, we present detailed descriptions of changes (and new insights) below.


\section*{\uppercase\expandafter{\romannumeral2.}\quad RESPONSE TO REVIEWER 1}

\noindent \textbf{Comment (Reviewer1.R1):} \textit{Clarify and demonstrate the theory and the performance for point queries.}

\noindent \textbf{Response:} Thank you for your comment. Regarding theoretical guarantees for point queries, we treat them as range queries in the interval that encompass only the corresponding data point. Thus our theoretical findings \emph{directly} apply to point queries. We discuss this in Section~\ref{section:point_queries}. Additionally, the empirical (accuracy) performance of \name on point queries is shown at the end of Section~\ref{section.exp.accuracy}. The results confirm that \name enhances the OOD robustness of MSCN for point queries.

\medskip
\noindent \textbf{Comment (Reviewer1.R2):} \textit{Clarify the theoretical guarantee on other OOD scenarios, including changes in the query structure and underlying dataset.}

\noindent \textbf{Response:} Thanks for pointing out this area of improvement. We have addressed the issue of changes in query structure under ``Scenario 3'' in Section~\ref{section.ood.cases}: ``When the join graph remains unchanged, adding or dropping predicates essentially changes the query granularity, therefore reducing to Scenario 2. Our theory does not support changes in the join graph as both Thm~\ref{theorem.remove.validity} and Thm~\ref{thm: ood} hold for each join graph \emph{independently}. Developing unified error bounds for all join graphs is promising future work.''

Regarding changes in the underlying dataset (\textit{i.e.,} data distribution shifts), we have detailed relevant discussions in Section~\ref{section:data_shift}. Here, Proposition~\ref{proposition:data_shift} extends Theorem~\ref{thm: ood} to manage data distribution shifts by establishing that if the old data distribution and the new data distribution are close in terms of the \emph{total variation distance}, then the OOD generalization error remains bounded. We are hopeful that in future work, this result can be improved; however, data distribution shifts are beyond the primary scope of this paper, and we consider it an area for future research.

\medskip
\noindent \textbf{Comment (Reviewer1.R3):} \textit{Clarify the specific guarantees that NeuroCDF and SeConCDF provide.}

\noindent \textbf{Response:} Thanks. We have expanded the discussion about specific guarantees of \textsc{NeuroCDF} in the ``Theoretical Guarantees'' subsection of Section~\ref{section.neurocdf.overview}: ``\neucdf, as a framework, can be proved to be induced by signed measures through its CDF modeling. Hence, both the in-distribution (Thm~\ref{theorem.remove.validity}) and OOD (Thm~\ref{thm: ood}) generalization error bounds \emph{directly} apply to \neucdf. This means given sufficient training queries and under Assumption \ref{assump: bdd}-\ref{assump: samp_R}, the in-distribution and OOD generalization errors of \neucdf are both close to its training error.''

We have also expanded the discussion about specific guarantees of \name at the end of  Section~\ref{section.secon.overview}:
``Although \name is inspired by both the theoretical and empirical analyses of \neucdf, it does not come with a theoretical guarantee because \emph{it cannot be confirmed as being entirely induced by signed measures}. Despite this, \name shows significant practical effectiveness in our experiments.''

\medskip
\noindent \textbf{Comment (Reviewer1.R4):} \textit{Clarify the theoretical properties of the four categories of query-driven approaches on their monotonicity and additivity.}

\noindent \textbf{Response:} Thank you for the comment. We have provided the theoretical analysis of the four categories of query-driven approaches on their monotonicity and additivity in the ``Theoretical Characteristics'' subsection of Section~\ref{section.gap}. Indeed, we found that these characteristics can be thoroughly analyzed theoretically. Consequently, due to space constraints, we have removed the empirical evaluations featured in the first draft (which are no longer necessary given the theoretical results). Additionally, there was a typo in Table~\ref{table.check} --- LEO indeed preserves additivity. Thank you again for the insightful suggestion!

\section*{\uppercase\expandafter{\romannumeral3.}\quad RESPONSE TO REVIEWER 2}


\noindent \textbf{Comment (Reviewer2.R1):} \textit{Add implementation details for proposed methods: give details such as how to combine a cumulative distribution function (CDF) with a query-based model for selective estimation, and a step-by-step explanation of data preprocessing, model training, and prediction steps.}

\noindent \textbf{Response:} Thank you for your comment. We have \emph{significantly} revised both Section~\ref{section.neucdf} and Section~\ref{section.training} to enhance the presentation of implementation details for \neucdf and \name, respectively. For \neucdf, detailed \emph{step-by-step} instructions are available in the ``Workflow of \textsc{NeuroCDF}'' subsection of Section~\ref{section.neurocdf.overview}, including normalization, CDF conversion, model training, and prediction. For \name, comprehensive procedural details are provided in Section~\ref{section.secon.cdf}, which include loss computation with query workload, loss computation with query generator, model training, and prediction processes. These enhancements aim to improve the reproducibility of our methods. Additionally, all code necessary for reproducing our results is provided (the code and data for new experiments in the revision will also be polished and uploaded), which could support the reproducibility of our work.

\medskip
\noindent \textbf{Comment (Reviewer2.R2):} \textit{Extensive experimental evaluation: reports on inference and training times for models, and adds other comparative methods that also address generalization problems. Test the model on more real-world data sets and scenarios to better understand the robustness and generalization of the model.}

\noindent \textbf{Response:} Thank you for your comment. For \textbf{inference and training times,} we have included the training and inference times for \name in Section~\ref{section.exp.efficiency}. While the training overheads (50s for IMDb-small, 26s for DSB, and 63s for CEB per epoch) of \name are higher than those for the original MSCN (14s, 8s, and 35s respectively, not reported in the paper due to space constraints), they are still not costly. More importantly, since \name \emph{does not change the model architecture or inference procedure} of MSCN, the inference time (which is more crucial for real query performance) for MSCN trained with \name  remains efficient and \emph{negligible} compared to the actual query execution time for complex join queries.
We have not included the training and inference times for \neucdf since we only conducted a preliminary evaluation of \neucdf using single-table data.  This is because \neucdf is not compatible with Qerror or MSLE as loss functions, as it may produce negative estimates (as detailed in the ``Limitation of \textsc{NeuroCDF}'' subsection of Section~\ref{section.neurocdf.theory}). Consequently, we focused primarily on conducting accuracy and query latency experiments for \name across various real-world datasets, as detailed in Section~\ref{section.eval}, since \name is a more general improvement strategy compatible with Qerror or MSLE. Nonetheless, this does not diminish the value of \neucdf, as both its theoretical and empirical analyses have shaped the design of \name. Moreover, \neucdf is provably supported by the theoretical guarantees of our theory. Hence, we hope to further improve \neucdf in future work by alleviating the negative estimate issue.

% due to our predominant use of \name in practice (as presented in Section~\ref{section.eval}) instead of \neucdf. This is because \neucdf is not compatible with Qerror or MSLE as loss functions (as detailed in the ''Limitation of \textsc{NeuroCDF}'' subsection of Section~\ref{section.neurocdf.theory}), which we hope to address in future work. However, as discussed in Section~\ref{section.secon.overview}, the theoretical and empirical analyses of \neucdf inspire the design of \name, which we implement for both accuracy and query latency experiments across different real-world datasets.

\textbf{New dataset and scenario.}  Additionally, as outlined in the ``Datasets'' and ``Workloads'' subsections of Section~\ref{section.exp.setup}, we have introduced a new real-world dataset (CEB) and a complex scenario (CEB-1a-varied) to better assess the robustness and generalization capabilities of the model. Specifically, unlike IMDb-small used in our initial draft, which uses 6 tables from the original IMDb, CEB incorporates 15 tables, enriching our evaluation with \emph{more diverse data}. Moreover, CEB-1a-varied includes 9-way join queries, including star queries, chain queries, and self-joins. These are significantly more intricate than the 5-way star joins in the benchmarks for our initial draft. This represents \emph{a new and more challenging scenario}. Consistent with our expectations, and as detailed in our response to Reviewer3.R3, our findings indicate consistent enhancements of \name across this new dataset and scenario. 

\textbf{Comparison with Robust-MSCN.} For another comparative method addressing generalization, we have included Robust-MSCN, as described in the ``Compared Approaches'' subsection of Section~\ref{section.exp.setup}. Due to space constraints, we report its results over the new CEB-1a-varied dataset, which features the most complex joins and presents a significant challenge for query optimization, making it more critical for evaluation. (We also observed consistent trends across other datasets, which we hope to present in a longer technical report in the future.) The detailed comparison with Robust-MSCN is provided in the ``Comparison with Robust-MSCN'' subsection (Table~\ref{table.ceb.qerror}) of Section~\ref{section.exp.accuracy} and the ``More joins'' subsection (Figure~\ref{fig:ceb_qo}) of Section~\ref{section.exp.e2e}, focusing on accuracy and latency performance, respectively. Overall, we found that \name outperforms Robust-MSCN in enhancing MSCN's OOD performance. However, it is important to note that this is because  Robust-MSCN is tailored for \emph{different OOD scenarios} like new join templates and missing tables/columns, which differ from the OOD scenarios (query center move and query granularity shift) that our theory addresses. Thank you for pointing out this comparative  approach as it deepens our understanding of how \name differs from existing approaches!


\medskip
\noindent \textbf{Comment (Reviewer2.R3):} \textit{Presentation Improvements: introduce some background information for PAC learning or measure theory, and make the theoretical part of the paper easy to understanding. Also need to correct presentation problems in the text to ensure consistency and clarity for readers.}

\noindent \textbf{Response:} Thank you for your comment. For \textbf{background information}, we have \emph{extensively} revised Section~\ref{subsec: sgn_m} and Section~\ref{subsec: PAC} to provide a more comprehensive background on measure theory and PAC learning, respectively. While  we strive to make these abstract mathematical concepts \emph{as accessible and intuitive as} possible, we concede that their complexity inherently limits the depth of explanation feasible in the Background section of a 12-page paper. To aid understanding of measure theory,  we relocated Example~\ref{example.measure}, which illustrates selectivity functions and their corresponding measures that induce them, to Section~\ref{subsec: sgn_m}. We have also divided the measure theory content into ``Basic Concepts'' and ``Advanced Concepts,'' allowing first-time readers to skip the more complex parts.
Similarly, for PAC learning, readers new to the topic can refer to Table~\ref{tab:term.summary} for a concise summary of essential concepts and may opt to skip more advanced topics like VC dimension and Fat-Shattering dimension if desired.

\textbf{Making our theory easier to understand.} In the theoretical part of the paper, we designed Section~\ref{section.theory.summary} to help readers grasp the main theoretical ideas intuitively. Additionally, in Section~\ref{section.ood}, where we discuss our main OOD generalization theorem (Thm~\ref{thm: ood}), we provide intuitive explanations for all relevant assumptions (Assumptions \ref{assump: bdd}-\ref{assump: samp_R}) and offer detailed justifications for each step in the proof. 
In this revision, to make our main theorem easier to understand, we have also included informal, high-level explanations below Thm~\ref{thm: ood} to make the theorem more approachable. 

We hope all these efforts can make PAC learning, measure theory, and the theoretical part of the paper easier to understand!

\textbf{Textual issues and inconsistencies.} For the presentation problems in the text, we have corrected the typo in ``We aim to answer \sout{three} two research questions as follows.'' Additionally, we have conducted another thorough proofreading of the paper to ensure consistency and clarity.

\section*{\uppercase\expandafter{\romannumeral4.}\quad RESPONSE TO REVIEWER 3}

\noindent \textbf{Comment (Reviewer3.R1):} \textit{``Is it possible to adapt the NeuroCDF approach (rectangle query) to other models (e.g., XGBoost) that might be simpler and/or more interpretable? Why are neural networks necessarily the right choice here?''}

\noindent \textbf{Response:} Thank you for the insightful question. We now discuss this in the ``Model Choice for CDF Prediction'' subsection of Section~\ref{section.neucdf.convert}. We summarize the discussion here for easy reference. We agree that using other non-NN models (\textit{e.g.,} XGBoost) as the CDF prediction model would be simpler and more interpretable. 

However, we opt for NNs due to their \emph{ease of optimization} in our setting. Specifically, XGBoost relies on direct mappings from data points to their CDF values (\(\mathbf{x} \mapsto F(\mathbf{x})\)) and optimizes based on gradients 
between predictions and actual values. However, in selectivity learning, we \emph{only} have mappings from queries to their selectivities (\(q \mapsto S(q)\)), lacking the direct data-to-CDF mappings (or actual CDF values) required by XGBoost. This makes optimizing XGBoost challenging. NNs, on the other hand, can be trained \emph{end-to-end} effectively using only \(q \mapsto S(q)\) mappings. Because the computation in Eq.~\ref{eq.cdf} is fully differentiable, we can employ backpropagation without needing direct \(\mathbf{x} \mapsto F(\mathbf{x})\) mappings (or the actual values of $F(\mathbf{x})$).

\medskip

\noindent \textbf{Comment (Reviewer3.R2):} \textit{``For Section 7.2 (Query Latency Performance), it would be helpful to include per-query metrics rather than (or in addition to) overall runtime, e.g., box plot of average speedup per query.''}

\noindent \textbf{Response:}
Thank you, we have provided per-query metrics along with overall running times for our new experiments on CEB (detailed in our response to Reviewer2.R2) within the ``More Joins'' subsection of Section~\ref{section.exp.e2e}, with the corresponding box plots shown in Figure~\ref{fig:ceb_qo}. Due to space constraints, we are unable to feature per-query plots for all datasets. Consequently, we opted to include the per-query plots for the CEB-1a-varied workload (as discussed in our response to Reviewer3.R3) under granularity shift (where a similar trend was observed for center move), which involves the \emph{most joins} (\textit{i.e., }9) and thus presents more significant challenges in query optimization.

Additionally, we highlight that \name significantly reduces MSCN's running time by at least a factor of two in 4 of the 20 OOD queries, without any notable regressions. This improvement is consistent across different sets of randomly sampled query workloads. Therefore, we believe the results clearly demonstrate that the improvements are not limited to a single query.


\medskip
\noindent \textbf{Comment (Reviewer3.R3):} \textit{Expand the evaluation to include larger numbers of joins, which is when traditional cardinality estimation methods tend to break down.}

\noindent \textbf{Response:} Thank you for your comment. We have expanded the evaluation in the revision to include scenarios with a larger number of joins. As detailed in the ``Workloads'' subsection of Section~\ref{section.exp.setup}, we have generated a new 9-way join query workload, CEB-1a-varied from CEB-1a. This was necessary because the original CEB-1a queries did not vary sufficiently in predicate values and thus did not meet the assumptions required for our theory. Therefore, the maximum number of joins evaluated in this revision has \emph{nearly doubled} compared to the original maximum of five joins considered in the first draft. We will include a more comprehensive set of benchmarks containing large numbers of joins in a future technical report. However, due to space constraints, we believe that CEB-1a-varied would be sufficient for the scope of this paper.

We present the accuracy performance and query latency performance in the ``More Joins'' subsections of Sections~\ref{section.exp.accuracy} and ~\ref{section.exp.e2e}, respectively. First, we did observe that all MSCN models outperform \pg in query latency on CEB-1a-varied by a large margin, because larger numbers of joins are usually when traditional cardinality estimation methods start to break down (as noted in the comment). Moreover, our results indicate that \name significantly improves MSCN’s OOD performance, enhancing both accuracy and query latency, despite the increased complexity introduced by the larger number of joins.


